Distributed Black-Box Optimization via Error Correcting Codes

We introduce a novel distributed derivative-free optimization framework that is resilient to stragglers. The proposed method employs coded search directions at which the objective function is evaluated, and a decoding step to find the next iterate. Our framework can be seen as an extension of evolution strategies and structured exploration methods where structured search directions were utilized. As an application, we consider black-box adversarial attacks on deep convolutional neural networks. Our numerical experiments demonstrate a significant improvement in the computation times.

==> least_squares.tex <==
\subsection{Case Study: $l_2$-Norm Squared Function}
We will show that, as a case study, when we consider the $l_2$-norm squared function $f(\theta)=\frac{1}{2}||A\theta - b||_2^2$, the gradient estimates become linear in perturbation directions. Hence the gradient estimates become the same as exact gradients. The term $f(\theta + \theta_1) - f(\theta - \theta_1)$ can be be simplified as follows when $f(.)$ is $l_2$-norm squared:
\begin{align}
    f(\theta + \theta_1) - f(\theta - \theta_1) &= 2\theta^TA^TA\theta_1 - 2b^TA\theta_1 \nonumber \\
    &= (2\theta^TA^TA - 2b^TA)\theta_1 \nonumber \\
    &= \theta_1^T (2A^TA\theta - 2A^Tb)
\end{align}
We note that the RHS is linear in $\theta_1$. Similarly, for $\theta_2$, we have
\begin{align}
    f(\theta + \theta_2) - f(\theta - \theta_2) &= \theta_2^T (2A^TA\theta - 2A^Tb).
\end{align}
We see that gradient estimates are linear in perturbation directions $\theta_1$ and $\theta_2$.
%It is now straightforward to see that the conditions in \eqref{decoding_conditions} are satisfied for $f(\theta)=||A\theta-b||_2^2$.
